Higher-Matter and Landau-Ginzburg Theory of Higher-Group Symmetries

Higher-matter is defined by higher-representation of a symmetry algebra, such as the $p$-form symmetries, higher-group symmetries or higher-categorical symmetries. In this paper, we focus on the cases of higher-group symmetries, which are formulated in terms of the strictification of weak higher-groups. We systematically investigate higher-matter charged under 2-group symmetries, defined by automorphism 2-representations. Furthermore, we construct a Lagrangian formulation of such higher-matter fields coupled to 2-group gauge fields in the path space of the spacetime manifold. We interpret such model as the Landau-Ginzburg theory for 2-group symmetries, and discuss the spontaneous symmetry breaking (SSB) of 2-group symmetries under this framework. Examples of discrete and continuous 2-groups are discussed. Interestingly, we find that a non-split 2-group symmetry can admit an SSB to a split 2-group symmetry, where the Postnikov class is trivialized. We also briefly discuss the strictification of weak 3-groups, weak 3-group gauge fields and 3-representations in special cases.

==> C2.tex <==

\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt     

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,1625); %set diagram left start at 0, and has height of 1625

%Curve Lines [id:da27899025227799146] 
\draw    (314,1514) .. controls (290.24,1470.44) and (361.55,1470) .. (336.78,1514.63) ;
\draw [shift={(336,1516)}, rotate = 300.41] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Curve Lines [id:da9070295596193472] 
\draw    (321,1455) .. controls (317.04,1422.33) and (337.58,1404.36) .. (334.11,1454.46) ;
\draw [shift={(334,1456)}, rotate = 274.4] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da9243890805236494] 
\draw    (231,1438.5) -- (259,1438.5) -- (292,1438.5)(231,1441.5) -- (259,1441.5) -- (292,1441.5) ;
\draw [shift={(300,1440)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Curve Lines [id:da5688627408762077] 
\draw    (199,1455) .. controls (195.04,1422.33) and (215.58,1404.36) .. (212.11,1454.46) ;
\draw [shift={(212,1456)}, rotate = 274.4] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

% Text Node
\draw (314,1506) node [anchor=north west][inner sep=0.75pt]    {$A$};
% Text Node
\draw (195,1458) node [anchor=north west][inner sep=0.75pt]    {$G$};
% Text Node
\draw (300,1457) node [anchor=north west][inner sep=0.75pt]    {$Aut( A)$};
% Text Node
\draw (318,1392) node [anchor=north west][inner sep=0.75pt]    {$A^{\times }$};
% Text Node
\draw (196,1396) node [anchor=north west][inner sep=0.75pt]    {$H$};
% Text Node
\draw (252,1409) node [anchor=north west][inner sep=0.75pt]    {$\mathcal{R}$};


\end{tikzpicture}


==> D1.tex <==


\begin{figure}[htbp]
    \centering
    \tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        
\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,1889); %set diagram left start at 0, and has height of 1889

%Curve Lines [id:da9980462247945963] 
\draw    (26,1693) .. controls (66,1663) and (109,1799) .. (179,1744) ;
%Straight Lines [id:da336197287241776] 
\draw [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ][line width=3.75]    (67,1704) -- (106,1741) ;
%Straight Lines [id:da7156701261159217] 
\draw    (195,1731) -- (256,1731) ;
\draw [shift={(258,1731)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Curve Lines [id:da10325712164439449] 
\draw    (293,1692) .. controls (333,1662) and (376,1798) .. (446,1743) ;
%Straight Lines [id:da7944823918109987] 
\draw [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ][line width=3.75]    (356,1682) -- (395,1719) ;
%Straight Lines [id:da7055894576698138] 
\draw [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ][line width=2.25]    (378,1743) -- (395,1719) ;
%Straight Lines [id:da1495711956605772] 
\draw [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ][line width=2.25]    (336,1707) -- (356,1682) ;
%Curve Lines [id:da42756420679367046] 
\draw [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ][line width=3]    (293,1692) .. controls (307,1682) and (317,1687) .. (336,1707) ;
%Curve Lines [id:da9931475909572691] 
\draw [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ][line width=3]    (378,1743) .. controls (394,1762) and (434,1760) .. (446,1743) ;

% Text Node
\draw (49,1757) node [anchor=north west][inner sep=0.75pt]    {$( \sigma ,\sigma +\epsilon )$};
% Text Node
\draw (332,1667) node [anchor=north west][inner sep=0.75pt]    {$\mu $};


\end{tikzpicture}
    \caption{Caption}
    \label{fig:lineseg}
\end{figure}
